NusaCrowd: Open Source Initiative for Indonesian NLP Resources

We present NusaCrowd, a collaborative initiative to collect and unify existing resources for Indonesian languages, including opening access to previously non-public resources. Through this initiative, we have brought together 137 datasets and 118 standardized data loaders. The quality of the datasets has been assessed manually and automatically, and their value is demonstrated through multiple experiments. NusaCrowd's data collection enables the creation of the first zero-shot benchmarks for natural language understanding and generation in Indonesian and the local languages of Indonesia. Furthermore, NusaCrowd brings the creation of the first multilingual automatic speech recognition benchmark in Indonesian and the local languages of Indonesia. Our work strives to advance natural language processing (NLP) research for languages that are under-represented despite being widely spoken.

==> author.tex <==

{\small Samuel Cahyawijaya} \\ {\small HKUST} \And
{\small Holy Lovenia} \\ {\small affiliation} \And 
{\small Alham Fikri Aji} \\ {\small affiliation} \And 
{\small Genta Indra Winata} \\ {\small affiliation} \And 
{\small Bryan Wilie} \\ {\small affiliation} \AND

{\small Rahmad Mahendra} \\ {\small affiliation} \And 
{\small Christian Wibisono} \\ {\small affiliation} \And 
{\small Ade Romadhony} \\ {\small affiliation} \And 
{\small Karissa Vincentio} \\ {\small affiliation} \And
{\small Fajri Koto} \\ {\small affiliation} \And 
{\small Jennifer Santoso} \\ {\small affiliation} \AND 
{\small David Moeljadi} \\ {\small affiliation} \And 
{\small Cahya Wirawan} \\ {\small affiliation} \And 
{\small Frederikus Hudi} \\ {\small affiliation} \And
{\small Ivan Halim Parmonangan} \\ {\small affiliation} \And  
{\small Ika Alfina} \\ {\small affiliation} \And 
{\small Muhammad Satrio Wicaksono} \\ {\small affiliation} \AND 
{\small Ilham Firdausi Putra} \\ {\small affiliation} \and
{\small Samsul Rahmadani} \\ {\small affiliation} \And 
{\small Yulianti Oenang} \\ {\small affiliation} \And  
{\small Ali Akbar Septiandri} \\ {\small affiliation} \And 
{\small James Jaya} \\ {\small affiliation} \And 
{\small Kaustubh D. Dhole} \\ {\small affiliation} \And 
{\small Arie Ardiyanti Suryani} \\ {\small affiliation} \AND 
{\small Rifki Afina Putri} \\ {\small affiliation} \And 
{\small Dan Su} \\ {\small affiliation} \And 
{\small Keith Stevens} \\ {\small affiliation} \And 
{\small Made Nindyatama Nityasya} \\ {\small affiliation} \And 
{\small Muhammad Farid Adilazuarda} \\ {\small affiliation} \And 
{\small Ryan Ignatius} \\ {\small affiliation} \AND 
{\small Ryandito Diandaru} \\ {\small affiliation} \And 
{\small Tiezheng Yu} \\ {\small affiliation} \And 
{\small Vito Ghifari} \\ {\small affiliation} \And 
{\small Wenliang Dai} \\ {\small affiliation} \And 
{\small Yan Xu} \\ {\small affiliation} \AND 
{\small Dyah Inastra} \\ {\small affiliation} \And 
{\small Cuk Tho} \\ {\small affiliation} \And 
{\small Ichwanul Muslim Karo Karo} \\ {\small affiliation} \And 
{\small Tirana Noor Fatyanosa} \\ {\small affiliation} \And 
{\small Ziwei Ji} \\ {\small affiliation} \AND 
{\small Pascale Fung} \\ {\small affiliation} \And 
{\small Graham Neubig} \\ {\small affiliation} \And 
{\small Timothy Baldwin} \\ {\small affiliation} \And 
{\small Sebastian Ruder} \\ {\small affiliation} \And 
{\small Herry Sujaini} \\ {\small affiliation} \And 
{\small Sakriani Sakti} \\ {\small affiliation} \And 
{\small Ayu Purwarianti} \\ {\small affiliation} \And 
